Unital Dilations of Completely Positive Semigroups

Dilations of completely positive semigroups to endomorphism semigroups have been studied by numerous authors. Most existing dilation theorems involve a non-unital embedding, corresponding to the embedding of $B(H)$ as a corner of $B(K)$ for Hilbert spaces $H \subset K$. A 1986 paper of Jean-Luc Sauvageot shows how to achieve a unital dilation, but does not specify how to do so while also preserving continuity properties of the original semigroup. This thesis further develops Sauvageot's dilation theory in order to establish the existence of continuous unital dilations, and to explore connections with free probability.

==> thesisAbstract.tex <==
% Thesis Abstract by Dave Gaebler

Semigroups of completely positive maps arise naturally both in noncommutative stochastic processes and in the dynamics of open quantum systems.  Since its inception in the 1970's, the study of
completely positive semigroups has included among its
central topics the dilation of a completely positive semigroup to an endomorphism semigroup.  In quantum dynamics, this amounts to embedding a given open system inside some closed system, while in noncommutative probability, it corresponds to the construction of a Markov process from its transition probabilities.  In addition to the existence of dilations, one is interested in what properties of the original semigroup (unitality, various kinds of continuity) are preserved.

Several authors have proved the existence of dilations, but in general, the dilation achieved has been non-unital; that is, the unit of the original algebra is embedded as a proper projection in the dilation algebra.  A unique approach due to Jean-Luc Sauvageot overcomes this problem, but leaves unclear the continuity of the dilation semigroup.  The major purpose of this thesis, therefore, is to further develop Sauvageot's theory in order to prove the existence of continuous unital dilations.
This existence is proved in Theorem \ref{thmkahuna}, the central
result of the thesis.

The dilation depends on a modification of free probability theory, and in particular on a combinatorial property akin to free independence.  This property is implicit in some of Sauvageot's original calculations, but a secondary goal of this thesis is to present it as its own object of study, which we do in chapter \ref{chapliberation}.


==> thesisAck.tex <==
Whatever I have achieved in life has depended on the assistance of countless others.  For my mathematical development, I would like to thank my parents for teaching me both how to do math and how to enjoy it, and for their continuing encouragement after I left the nest.  Among my undergraduate mentors I especially remember Michael Moody, who convinced me to become a mathematician; Art Benjamin, who awakened me to the showmanship inherent in good mathematical exposition; and Francis Su, who showed me how to be wise as well as smart.  More recently, my advisor, Paul Muhly, has modeled the many dimensions of mathematical maturity; has been relentlessly encouraging at every step of my research, during both the discoveries and the setbacks; and has taken a sincere interest in my personal as well as professional well-being.  I truly cannot thank him enough.  Other mathematicians have been kind to me as well.  Most closely related to this thesis, Orr Shalit and Daniel Markiewicz have been patient in bringing me up to speed with the basics of CP-semigroups.  And fellow Muhly disciples Jonas, Andrew, Travis, Jenni, Erin, and Rachael formed the cadre of compatriots without which graduate school would be harder than it already is.

The support staff at the University of Iowa have rendered invaluable assistance, and I would like especially to thank Margaret Driscol, Cindy Farthing, and Lucy Silag for their courtesy, professionalism, and expertise.

\newpage

As much as I enjoy mathematics for its own sake, my toil under the sun is made meaningful by my family.  Two are indeed better than one, and a cord of five (so far!) strands is not easily broken.  My wife Leslie has gone out of her way to free up my time and to cheer me on, even while she has her hands full caring for $3-\epsilon$ small children.  An excellent wife is the crown of her husband, and my crown is more splendid than any man could deserve.  I would also like to thank my sons for their patience during my busy times, and my in-laws for helping cover all the bases.


Most of all, thanks are due to God the Father, in whom we live and move and have our being; the Son, in whom are hidden all the treasures of wisdom and knowledge; and the Spirit, who enables all skilled workmen from Bezalel to the present day.  SDG.


==> thesisDedication.tex <==
\begin{center}
Sicut lilium inter spinas,

\vspace{.5in}

sic amica mea inter filias
\end{center}

